Identifying the Discount Factor in Dynamic Discrete Choice Models

Empirical research often cites observed choice responses to variation that shifts expected discounted future utilities, but not current utilities, as an intuitive source of information on time preferences. We study the identification of dynamic discrete choice models under such economically motivated exclusion restrictions on primitive utilities. We show that each exclusion restriction leads to an easily interpretable moment condition with the discount factor as the only unknown parameter. The identified set of discount factors that solves this condition is finite, but not necessarily a singleton. Consequently, in contrast to common intuition, an exclusion restriction does not in general give point identification. Finally, we show that exclusion restrictions have nontrivial empirical content: The implied moment conditions impose restrictions on choices that are absent from the unconstrained model.

==> ddcGraphs.tex <==

% =================================================
% GRAPHS
% 	- data need to be created by running ddc.m with Matlab
% =================================================

%% Rust shape restriction
\begin{figure}[t]
\caption{Example of a Shape Restriction on Utility that Implies an Exclusion Restriction\label{fig:zurchercost}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=llherr,
        xlabel={miles},
        ylabel={$c(x)$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={1,2,3,4,5,6},
        xticklabels={$x_1$,$x_2$,$x_3$,$x_4$,$x_5$,$x_6$},
        ytick={0},
   %     ytick={0,2,4,6},
    %    yticklabels={$0$,$2$,$4$,$6$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=7,
	ymin=0,
	ymax=6,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \addplot[color=blue!75,mark=*,line width=0.75pt]  coordinates { (1,1) (2,1) (3,2) (4,4) (5,5) (6,5.5) };
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize Note: In this stylized example of \cites{ecta87:rust} bus engine renewal problem, mileage takes $J=6$ values, the cost $c(x)$ of operating an engine with $x$ miles is constant between $x_1$ and $x_2$ miles and increases thereafter, and the utility $u_1^*(x)$ from operating an engine with $x$ miles equals a constant minus the operating cost  $c(x)$.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example in Which an Exclusion Restriction on Current Values Suffices for Identification but One on Primitive Utility Does Not\label{fig:identificationFails}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=llherr,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\identificationFailsPreciseBetaOne,\identificationFailsPreciseBetaTwo},
        xticklabels={$0$,$\identificationFailsBetaOne$,$\identificationFailsBetaTwo$},
        ytick={0,\identificationFailsPreciseLhs},
        yticklabels={$0$,$\identificationFailsLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=black!75,line width=0.75pt,solid] (axis cs:0,\identificationFailsPreciseLhs) -- (axis cs:1,\identificationFailsPreciseLhs);
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt] table[x=beta,y=rhs,col sep=comma]{matlab/data/identificationFails.csv} ;
		\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\identificationFailsPreciseBetaOne,0) -- (axis cs:\identificationFailsPreciseBetaOne,\identificationFailsPreciseLhs);
         	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\identificationFailsPreciseBetaTwo,0) -- (axis cs:\identificationFailsPreciseBetaTwo,\identificationFailsPreciseLhs);
        	\addplot[color=red!75,dashed,mark=,line width=0.75pt] table[x=beta,y=rhsMT,col sep=comma]{matlab/data/identificationFails.csv} ;
        		\draw[color=red!75,line width=0.75pt,dotted] (axis cs:\identificationFailsPreciseBetaMT,0) -- (axis cs:\identificationFailsPreciseBetaMT,\identificationFailsPreciseLhs);
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize Note: For $J=\identificationFailsJ$ states, $K=\identificationFailsK$ choices, $k=l=1$, $\tilde{x}_1=x_1$, and $\tilde{x}_2=x_2$, this graph plots the left hand side of  (\ref{eq:diffMT})  and (\ref{eq:diffAD}) (solid black horizontal line) and the right hand sides of (\ref{eq:diffMT}) (dashed red line), and (\ref{eq:diffAD}) (solid blue curve) as functions of $\beta$. The data are $\mathbf{Q}_1(x_1)=\identificationFailsQiRowOne$, $\mathbf{Q}_1(x_2)=\identificationFailsQiRowTwo$,}

{\scriptsize 
\vspace*{-3ex} 
\[\mathbf{Q}_K=\identificationFailsQK\text{, }\mathbf{p}_1=\identificationFailsPOne\text{, and }\mathbf{p}_K=\identificationFailsPK.\] 

Consequently, the left hand side of (\ref{eq:diffMT})  and (\ref{eq:diffAD}) equals $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)= \identificationFailsLhs$. Moreover,  $\mathbf{m}'=\identificationFailsMPrime$ and $\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)=\identificationFailsDeltaQ$, so that the slope of the dashed red line equals $\left[\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)\right] \mathbf{m}=\identificationFailsDeltaQM$. A unique value of $\beta$,  $\identificationFailsBetaMT$, solves  (\ref{eq:diffMT}), but two values of  $\beta$ solve (\ref{eq:diffAD}): $\identificationFailsBetaOne$ and $\identificationFailsBetaTwo$.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example in Which \citeauthor{ecta02:magnacthesmar}'s Rank Condition Fails, but an Exclusion Restriction on Primitive Utility Suffices for Identification\label{fig:needNoMT}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=llherr,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\needNoMTPreciseBetaOne},
        xticklabels={$0$,$\needNoMTBetaOne$},
        ytick={0,\needNoMTPreciseLhs},
        yticklabels={$0$,$\needNoMTLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.1,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=black!75,line width=0.75pt,solid] (axis cs:0,\needNoMTPreciseLhs) -- (axis cs:1,\needNoMTPreciseLhs);
        	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\needNoMTPreciseBetaOne,0) -- (axis cs:\needNoMTPreciseBetaOne,\needNoMTPreciseLhs);
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt] table[x=beta,y=rhs,col sep=comma]{matlab/data/needNoMT.csv};
        	\addplot[color=red!75,dashed,mark=,line width=2pt] table[x=beta,y=rhsMT,col sep=comma]{matlab/data/needNoMT.csv};
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize Note: For $J=\needNoMTJ$ states, $K=\needNoMTK$ choices, $k=l=1$, $\tilde{x}_1=x_1$, and $\tilde{x}_2=x_2$, this graph plots the left hand side of  (\ref{eq:diffMT})  and (\ref{eq:diffAD}) (solid black horizontal line) and the right hand sides of (\ref{eq:diffMT}) (dashed red line) and (\ref{eq:diffAD}) (solid blue curve) as functions of $\beta$. The data are $\mathbf{Q}_1(x_1)=\needNoMTQiRowOne$, $\mathbf{Q}_1(x_2)=\needNoMTQiRowTwo$,}

{\scriptsize 
\vspace*{-3ex} 
\[\mathbf{Q}_K=\needNoMTQK\text{, }\mathbf{p}_1=\needNoMTPOne \text{, and }\mathbf{p}_K=\needNoMTPK.\] 

Consequently, the left hand side of (\ref{eq:diffMT})  and (\ref{eq:diffAD}) equals $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)= \needNoMTLhs$. Moreover,  $\mathbf{m}'=\needNoMTMPrime$ and $\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)=\needNoMTDeltaQ$, so that the slope of the dashed red line equals $\left[\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)\right] \mathbf{m}=\needNoMTDeltaQM$. A unique value of $\beta$,  $\needNoMTBetaOne$, solves  (\ref{eq:diffAD}), but (\ref{eq:diffMT}) has no solution.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example of Data that are Consistent with an Exclusion Restriction on Current Values but Not with One on Primitive Utility\label{fig:moreEmpiricalContent}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=llherr,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\moreEmpiricalContentPreciseBetaMT},
        xticklabels={$0$,$\moreEmpiricalContentBetaMT$},
        ytick={0,\moreEmpiricalContentPreciseLhs},
        yticklabels={$0$,$\moreEmpiricalContentLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=\moreEmpiricalContentMinRhs,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=black!75,line width=0.75pt,solid] (axis cs:0,\moreEmpiricalContentPreciseLhs) -- (axis cs:1,\moreEmpiricalContentPreciseLhs);
        \draw[color=black!75,line width=0.75pt,dashed] (axis cs:0,0) -- (axis cs:1,0);
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt] table[x=beta,y=rhs,col sep=comma]{matlab/data/moreEmpiricalContent.csv} ;
        	\addplot[color=red!75,dashed,mark=,line width=0.75pt] table[x=beta,y=rhsMT,col sep=comma]{matlab/data/moreEmpiricalContent.csv} ;
        	\draw[color=red!75,line width=0.75pt,dotted] (axis cs:\moreEmpiricalContentPreciseBetaMT,\moreEmpiricalContentMinRhs) -- (axis cs:\moreEmpiricalContentPreciseBetaMT,\moreEmpiricalContentPreciseLhs);
\end{axis}
\end{tikzpicture}
\medskip
\begin{minipage}{\figwidth}
{\scriptsize Note: For $J=\moreEmpiricalContentJ$ states, $K=\moreEmpiricalContentK$ choices, $k=l=1$, $\tilde{x}_1=x_1$, and $\tilde{x}_2=x_2$, this graph plots the left hand side of  (\ref{eq:diffMT})  and (\ref{eq:diffAD}) (solid black horizontal line) and the right hand sides of (\ref{eq:diffMT})  (dashed red line) and (\ref{eq:diffAD}) (solid blue curve) as functions of $\beta$. The data are $\mathbf{Q}_1(\tilde{x}_1)=\moreEmpiricalContentQiRowOne$, $\mathbf{Q}_1(\tilde{x}_2)=\moreEmpiricalContentQiRowTwo$,}

{\scriptsize 
\vspace*{-3ex} 
\[\mathbf{Q}_K=\moreEmpiricalContentQK\text{, }\mathbf{p}_1=\moreEmpiricalContentPOne\text{, and }\mathbf{p}_K=\moreEmpiricalContentPK.\] 

Consequently, the left hand side of (\ref{eq:diffMT})  and (\ref{eq:diffAD}) equals $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)= \moreEmpiricalContentLhs$. Moreover,  $\mathbf{m}'=\moreEmpiricalContentMPrime$ and $\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)=\moreEmpiricalContentDeltaQ$, so that the slope of the dashed red line equals $\left[\mathbf{Q}_1(x_1)-\mathbf{Q}_K(x_1)- \mathbf{Q}_1(x_2)+\mathbf{Q}_K(x_2)\right] \mathbf{m}=\moreEmpiricalContentDeltaQM$. A unique value of $\beta$,  $\moreEmpiricalContentBetaMT$, solves  (\ref{eq:diffMT}), but (\ref{eq:diffAD}) has no solution.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example with Two Moment Conditions of Which One Identifies the Discount Factor\label{fig:oneRedundant}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=llherr,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\oneRedundantOnePreciseBetaOne,\oneRedundantTwoPreciseBetaTwo},
        xticklabels={$0$,$\oneRedundantOneBetaOne$,$\oneRedundantTwoBetaTwo$},
        ytick={0,\oneRedundantOnePreciseLhs,\oneRedundantTwoPreciseLhs},
        yticklabels={$0$,$\oneRedundantOneLhs$,$\oneRedundantTwoLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.04,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=red!75,line width=0.75pt,dashed] (axis cs:0,\oneRedundantOnePreciseLhs) -- (axis cs:1,\oneRedundantOnePreciseLhs);
        \draw[color=blue!75,line width=0.75pt,solid] (axis cs:0,\oneRedundantTwoPreciseLhs) -- (axis cs:1,\oneRedundantTwoPreciseLhs);
        	\draw[color=black!75,line width=0.75pt,dotted] (axis cs:\oneRedundantOnePreciseBetaOne,0) -- (axis cs:\oneRedundantOnePreciseBetaOne,\oneRedundantOnePreciseLhs);
        	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\oneRedundantTwoPreciseBetaTwo,0) -- (axis cs:\oneRedundantTwoPreciseBetaTwo,\oneRedundantTwoPreciseLhs);
        \addplot[color=red!75,smooth,mark=,line width=0.75pt,dashed] table[x=beta,y=oneRhs,col sep=comma]{matlab/data/oneRedundant.csv};
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt,solid] table[x=beta,y=twoRhs,col sep=comma]{matlab/data/oneRedundant.csv};
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize Note:  For $J=\oneRedundantJ$ states, $K=\oneRedundantK$ choices, and $k=l=1$, this graph plots the left (horizontal lines) and right hand sides (curves) of (\ref{eq:diffAD}) as functions of $\beta$, for $\tilde x_1=x_1$ and $\tilde x_2=x_2$ (corresponding to $u_1(x_1) = u_1(x_2)$; dashed red) and $\tilde x_1=x_3$ and $\tilde x_2=x_4$ (corresponding to $u_1(x_3) = u_1(x_4)$; solid blue). The data are}

{\scriptsize 
\vspace*{-3ex} 
\[\mathbf{Q}_1 = \oneRedundantQi, \mathbf{Q}_K=\oneRedundantQK\text{, }\]
\[\mathbf{p}_1^\prime=\oneRedundantPOne \text{, and }\mathbf{p}_K^\prime=\oneRedundantPK.\] 

Consequently, the left hand sides of (\ref{eq:diffAD}) equal $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)= \oneRedundantOneLhs$ and $\ln\left(p_1(x_3)/p_K(x_3)\right) - \ln\left(p_1(x_4)/p_K(x_4)\right)= \oneRedundantTwoLhs$. A unique value of $\beta$, $\oneRedundantOneBetaOne$, solves (\ref{eq:diffAD}) for $\tilde x_1=x_1$ and $\tilde x_2=x_2$  (dashed red). Two values of $\beta$ solve  (\ref{eq:diffAD}) for $\tilde x_1=x_3$ and $\tilde x_2=x_4$ (solid blue), of which one coincides with the solution to the first moment condition.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example with Two Moment Conditions that Jointly Identify the Discount Factor but Individually Do Not\label{fig:twiceTwo}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=mom,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\twiceTwoOnePreciseBetaOne,\twiceTwoOnePreciseBetaTwo,\twiceTwoTwoPreciseBetaOne},
        xticklabels={$0$,$\twiceTwoOneBetaOne$,$\twiceTwoOneBetaTwo$,$\twiceTwoTwoBetaOne$},
        ytick={0,\twiceTwoOnePreciseLhs,\twiceTwoTwoPreciseLhs},
        yticklabels={$0$,$\twiceTwoOneLhs$,$\twiceTwoTwoLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.015,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=red!75,line width=0.75pt,dashed] (axis cs:0,\twiceTwoOnePreciseLhs) -- (axis cs:1,\twiceTwoOnePreciseLhs);
        \draw[color=blue!75,line width=0.75pt,solid] (axis cs:0,\twiceTwoTwoPreciseLhs) -- (axis cs:1,\twiceTwoTwoPreciseLhs);
        	\draw[color=black!75,line width=0.75pt,dotted] (axis cs:\twiceTwoOnePreciseBetaTwo,0) -- (axis cs:\twiceTwoOnePreciseBetaTwo,\twiceTwoOnePreciseLhs);
        	\draw[color=red!75,line width=0.75pt,dotted] (axis cs:\twiceTwoOnePreciseBetaOne,0) -- (axis cs:\twiceTwoOnePreciseBetaOne,\twiceTwoOnePreciseLhs);
        	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\twiceTwoTwoPreciseBetaOne,0) -- (axis cs:\twiceTwoTwoPreciseBetaOne,\twiceTwoTwoPreciseLhs);
        \addplot[color=red!75,smooth,mark=,line width=0.75pt,dashed] table[x=beta,y=oneRhs,col sep=comma]{matlab/data/twiceTwo.csv};
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt,solid] table[x=beta,y=twoRhs,col sep=comma]{matlab/data/twiceTwo.csv};
\end{axis}

\path(mom.origin) ++(0,-2.7in) coordinate (crit plot position);
\begin{axis}[width=\figwidth,height=\figheight,
        name=crit,
        at = {(crit plot position)},
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\twiceTwoOnePreciseBetaTwo},
        xticklabels={$0$,$\twiceTwoOneBetaTwo$},
        ytick={0,0.5},
        yticklabels={$0$,$0.50$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.74,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \addplot[color=black!75,smooth,mark=,line width=0.75pt,solid] table[x=beta,y=quadDist,col sep=comma]{matlab/data/twiceTwo.csv};             
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize 
Note: For $J=\twiceTwoJ$ states, $K=\twiceTwoK$ choices, and $k=l=1$, the graph in the top panel plots the left (horizontal lines) and right hand sides (curves) of (\ref{eq:diffAD}) as functions of $\beta$, for $\tilde x_1=x_1$ and $\tilde x_2=x_2$ (corresponding to $u_1(x_1) = u_1(x_2)$; dashed red) and $\tilde x_1=x_3$ and $\tilde x_2=x_4$ (corresponding to $u_1(x_3) = u_1(x_4)$; solid blue). The graph in the bottom panel plots the corresponding squared Euclidian distance between the left and right hand sides of (\ref{eq:diffAD}) as a function of $\beta$ (in multiples of $10^{-\twiceTwoNoiseDistScaler}$). The data are}

{\scriptsize 
\vspace*{-3ex}
\[\mathbf{Q}_1 = \twiceTwoQi,~ \mathbf{Q}_K=\twiceTwoQK,\]
\[\mathbf{p}_1^\prime=\twiceTwoPOne\text{, and }\mathbf{p}_K^\prime=\twiceTwoPK.\]

Consequently, the left hand sides of (\ref{eq:diffAD}) equal $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)= \twiceTwoOneLhs$ and $\ln\left(p_1(x_3)/p_K(x_3)\right) - \ln\left(p_1(x_4)/p_K(x_4)\right)= \twiceTwoTwoLhs$. A unique value of $\beta$, $\twiceTwoOneBetaTwo$, solves  (\ref{eq:diffAD}) for both $\tilde x_1=x_1$ and $\tilde x_2=x_2$ (dashed red) and $\tilde x_1=x_3$ and $\tilde x_2=x_4$ (solid blue). In addition, each of these two moment condition has one other solution.}
\end{minipage}
\end{figure}

%% =======
\begin{figure}[t]
\caption{Example with Two Moment Conditions that Jointly Identify the Discount Factor but Individually Do Not, Using Noisy Estimates of the Choice Probabilities\label{fig:twiceTwoNoise}}
\medskip
\begin{tikzpicture}
   \begin{axis}[width=\figwidth,height=\figheight,
        name=noisyMom,
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\twiceTwoNoiseOnePreciseBetaOne,\twiceTwoNoiseOnePreciseBetaTwo,\twiceTwoNoiseTwoPreciseBetaOne,\twiceTwoNoiseTwoPreciseBetaTwo},
        xticklabels={$0$,$\twiceTwoNoiseOneBetaOne$,$\twiceTwoNoiseOneBetaTwo$,$\twiceTwoNoiseTwoBetaOne$,$\twiceTwoNoiseTwoBetaTwo$},
        ytick={0,\twiceTwoNoiseOnePreciseLhs,\twiceTwoNoiseTwoPreciseLhs},
        yticklabels={$0$,$\twiceTwoNoiseOneLhs$,$\twiceTwoNoiseTwoLhs$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.015,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=red!75,line width=0.75pt,dashed] (axis cs:0,\twiceTwoNoiseOnePreciseLhs) -- (axis cs:1,\twiceTwoNoiseOnePreciseLhs);
        \draw[color=blue!75,line width=0.75pt,solid] (axis cs:0,\twiceTwoNoiseTwoPreciseLhs) -- (axis cs:1,\twiceTwoNoiseTwoPreciseLhs);
        	\draw[color=red!75,line width=0.75pt,dotted] (axis cs:\twiceTwoNoiseOnePreciseBetaOne,0) -- (axis cs:\twiceTwoNoiseOnePreciseBetaOne,\twiceTwoNoiseOnePreciseLhs);	
	\draw[color=red!75,line width=0.75pt,dotted] (axis cs:\twiceTwoNoiseOnePreciseBetaTwo,0) -- (axis cs:\twiceTwoNoiseOnePreciseBetaTwo,\twiceTwoNoiseOnePreciseLhs);
        	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\twiceTwoNoiseTwoPreciseBetaOne,0) -- (axis cs:\twiceTwoNoiseTwoPreciseBetaOne,\twiceTwoNoiseTwoPreciseLhs);
        	\draw[color=blue!75,line width=0.75pt,dotted] (axis cs:\twiceTwoNoiseTwoPreciseBetaTwo,0) -- (axis cs:\twiceTwoNoiseTwoPreciseBetaTwo,\twiceTwoNoiseTwoPreciseLhs);
        \addplot[color=red!75,smooth,mark=,line width=0.75pt,dashed] table[x=beta,y=oneRhs,col sep=comma]{matlab/data/twiceTwoNoise.csv};
        \addplot[color=blue!75,smooth,mark=,line width=0.75pt,solid] table[x=beta,y=twoRhs,col sep=comma]{matlab/data/twiceTwoNoise.csv};
\end{axis}

\path(noisyMom.origin) ++(0,-2.7in) coordinate (noisyCrit plot position);
\begin{axis}[width=\figwidth,height=\figheight,
        name=noisyCrit,
        at = {(noisyCrit plot position)},
        xlabel={$\beta$},
        axis x line=bottom,
        every outer x axis line/.append style={-,color=gray,line width=0.75pt},
        axis y line=left,
        every outer y axis line/.append style={-,color=gray,line width=0.75pt},
        xtick={0,\twiceTwoNoisePreciseBetaSetOne,\twiceTwoNoisePreciseBetaSetTwo,\twiceTwoNoisePreciseBetaSetThree,\twiceTwoNoisePreciseBetaSetFour},
        xticklabels={$0$,$\twiceTwoNoiseBetaSetOne$,$\twiceTwoNoiseBetaSetTwo$,$\twiceTwoNoiseBetaSetThree$,$\twiceTwoNoiseBetaSetFour$},
        ytick={0,\twiceTwoNoisePreciseCriticalValue,0.5},
        yticklabels={$0$,$s_n$,$0.50$},
        every tick/.append style={line width=0.75pt},
	xmin=0, 
	xmax=1,
	ymin=0,
	ymax=0.74,
        scaled ticks=false,
        /pgf/number format/precision=2,
        /pgf/number format/set thousands separator={}]
        \draw[color=black!75,line width=0.75pt,solid] (axis cs:0,\twiceTwoNoisePreciseCriticalValue) -- (axis cs:1,\twiceTwoNoisePreciseCriticalValue);
        \addplot[color=black!75,smooth,mark=,line width=0.75pt,solid] table[x=beta,y=quadDist,col sep=comma]{matlab/data/twiceTwoNoise.csv};             
	\addplot [line width=0.75pt,color=green!75,mark=,fill=green, fill opacity=0.05]coordinates {
		(\twiceTwoNoisePreciseBetaSetOne, 0) 
		(\twiceTwoNoisePreciseBetaSetTwo, 0) 
            	(\twiceTwoNoisePreciseBetaSetTwo,\twiceTwoNoisePreciseCriticalValue)  
           	(\twiceTwoNoisePreciseBetaSetOne,\twiceTwoNoisePreciseCriticalValue)
                 (\twiceTwoNoisePreciseBetaSetOne, 0) };
	\addplot [line width=0.75pt,color=green!75,mark=,fill=green, fill opacity=0.05]coordinates {
		(\twiceTwoNoisePreciseBetaSetThree, 0) 
		(\twiceTwoNoisePreciseBetaSetFour, 0) 
            	(\twiceTwoNoisePreciseBetaSetFour,\twiceTwoNoisePreciseCriticalValue)  
           	(\twiceTwoNoisePreciseBetaSetThree,\twiceTwoNoisePreciseCriticalValue)
                 (\twiceTwoNoisePreciseBetaSetThree, 0) };
\end{axis}
\end{tikzpicture}
\medskip

\begin{minipage}{\figwidth}
{\scriptsize Note: This figure redraws Figure \ref{fig:twiceTwo} for the same values of $\mathbf{Q}_1$ and $\mathbf{Q}_K$, but randomly perturbed values of its choice probabilities $\mathbf{p}_1$ and $\mathbf{p}_K$. Rounded to two digits, the perturbed choice probabilities equal those reported below Figure \ref{fig:twiceTwo}. Consequently, the perturbation to $\mathbf{m}=-\ln\mathbf{p}_K$ is very small too, so that  the right hand sides of  (\ref{eq:diffAD}) are very close to those plotted in Figure \ref{fig:twiceTwo}. The left hand sides of (\ref{eq:diffAD}), however, now equal $\ln\left(p_1(x_1)/p_K(x_1)\right) - \ln\left(p_1(x_2)/p_K(x_2)\right)=\twiceTwoNoiseOneLhs$ (instead of $\twiceTwoOneLhs$) and $\ln\left(p_1(x_3)/p_K(x_3)\right) - \ln\left(p_1(x_4)/p_K(x_4)\right)= \twiceTwoNoiseTwoLhs$ (instead of $\twiceTwoTwoLhs$). The resulting moment conditions again have two solutions. However, they no longer share a common solution and the squared Euclidian distance in the bottom panel never attains zero. The green shaded areas highlight the intervals $[\twiceTwoNoiseBetaSetOne,\twiceTwoNoiseBetaSetTwo]$ and $[\twiceTwoNoiseBetaSetThree,\twiceTwoNoiseBetaSetFour]$ of values of $\beta$ at which the distance is below some critical level $s_n$ (which is taken to be $\twiceTwoNoiseCriticalValue\times 10^{-\twiceTwoNoiseDistScaler}$ in this example).}
\end{minipage}
\end{figure}


